Machine Learning Applications to Diffuse Reflectance Spectroscopy in Optical Diagnosis; A Systematic Review

Diffuse Reflectance Spectroscopy has demonstrated a strong aptitude for identifying and differentiating biological tissues. However, the broadband and smooth nature of these signals require algorithmic processing, as they are often difficult for the human eye to distinguish. The implementation of machine learning models for this task has demonstrated high levels of diagnostic accuracies and led to a wide range of proposed methodologies for applications in various illnesses and conditions. In this systematic review, we summarise the state of the art of these applications, highlight current gaps in research and identify future directions. This review was conducted in accordance with the PRISMA guidelines. 77 studies were retrieved and in-depth analysis was conducted. It is concluded that diffuse reflectance spectroscopy and machine learning have strong potential for tissue differentiation in clinical applications, but more rigorous sample stratification in tandem with in-vivo validation and explainable algorithm development is required going forward.

==> Notes.tex <==
\section{Colorectal Cancer}
\citet{saito_nogueira_insights_2022} used DRS to identify the main colorectal cancer biomarkers and developed a machine-learning model to permit the integration of DRS into medical devices. The authors found that the main differentiating biomolecules were oxy- and deoxy haemoglobin followed by water and lipid. The best wavelength ranges for classification differed by probing depth. The short-SDD probe, for superficial tissue, functioned best at 350-590nm and 600-1230nm and the long-SDD probe, for deeper tissue layers functioned best at 380-400 nm, 420-610 nm and 650-950 nm. Accuracies as high as 89.7\% were achieved (Sepcificity = 89.7, Sensitivity = 89.6, AUC = 0.96) using a KNN model.

\citet{nazarian_real-time_2024} proposed a DRS probe in combination with a real-time tracking system for the differentiation of cancerous and non-cancerous colorectal tissue. Human ex-vivo specimens were sampled directly after excision from 23 patients (17 male, 6 female). The highest classification accuracies were achieved using SpecNet, a neural network-based classifier (Accuracy = 0.91, Specificity = 0.88, Sensitivity = 0.93, AUC = 0.97). 

\citet{baltussen_tissue_2019} implemented an SVM to determine the added value of DRS for tissue characterization during colorectal cancer surgery in comparison to human judgment. Two binary comparisons were made; first, Fat vs. healthy and tumorous colorectal wall and second, tumour us. healthy colorectal wall. The SVM achieved accuracies of 0.92 (specificity = 0.94, sensitivity = 0. 89, MCC = 0.83) and 0. 89 (specificity = 0.87, Sensitivity = 0. 92, MCC = 0. 77) for each classification respectively. The authors conclude that DRS demonstrates strong potential for tissue classification during colorectal surgery, especially given the low false positive rates.

\citet{baltussen_diffuse_2017} used SVM to differentiate tumour tissue from healthy surrounding tissue in patients with colorectal neoplasia. Spectra from 38 patients were collected ex-vivo. The classifier was found to distinguish between healthy and cancerous tissue with high accuracies in both homogenous and inhomogeneous tissues. The overall achieved accuracy was 0. 95. The dataset was imbalanced at baseline with 63.4\% of samples belonging to the healthy class. The authors conclude that the results are promising but applications are still limited to the study's set-up and protocol. Future research should consider the feasibility of in-vivo implementation.

\citet{baltussen_optimizing_2019} attempted to identify the best method for the differentiation of healthy colorectal wall from tumour tissue. To this end, four normalisation techniques, four feature extraction techniques and five classifiers were implemented on nine datasets to obtain the optimal method for tissue differentiation. The best approach was found to be the application of feature extraction based on tissue optical features or shape-based features on SNV-normalised spectra and the classification via an SVM or a neural network classifier. It is interesting to note that this identified 'global optimum' is still outperformed by dataset-specific optimisation on seven of the nine datasets, indicating that changes in data-collection protocol yield large effects on the best structure of the implemented classifier and optimisation may be specific to datasets rather than datatypes.

\citet{nogueira_benefit_2021} evaluated the ability of an SVM to detect colorectal cancer in an extended DRS wavelength range of 350-1919 nm. Data was acquired from 47 subjects ex-vivo using freshly excised tissues. A total of 1363 spectra were collected, and using the full wavelength range, high classification accuracies were achieved (0.935 sensitivity, 0.94 specificity and 0.971 AUC). The authors conclude that future studies should use the broadband wavelength range. In addition, they argue that the fast processing times (2-3 seconds per spectra) may allow the integration of DRS into real-time surgery.

\citet{nogueira_evaluation_2021} investigated the difference in classification accuracy between a shallow and deep DRS probe for the diagnosis of colorectal cancer. A total of 2889 DRS spectra were collected from 47 patients between the ranges of 350 - 1919 nm To probe different tissue depths, source-detection distances of 630 µm and 2500 µm were tested. Using a quadratic SVM, 10-fold cross-validation demonstrated high results for both probes. The short-distance probe for superficial tissue demonstrated 0.935 sensitivity and 0.94 specificity. The long-distance probe for deeper tissue layers demonstrated 0.961 sensitivity and 0.957 specificity. From this, the authors concluded, that using a broader spectrum and longer near-infrared wavelengths may improve accuracies in detecting colorectal cancer and probe deeper tissue layers. 

\citet{nogueira_intestinal_2024} proposed the use of DRS to assist with anastomosis, the re-connecting of tissue after the removal of pathological tissue in the intestine and bowel area. The authors aim to classify fat, mucosa and muscle tissues to improve the potential of robotic surgery for the re-connection of tissue without the need for human tactile feedback. Two probe lengths were tested for this task and a quadratic SVM was used for the multiclass classification. The 630 µm probe for surface-level tissues achieved true positive rates of 0.979 for fat tissue, 0.955 for mucosa and 0.955 for muscle. The 2500 µm probe for deeper-level tissues achieved true positive rates of 0.967 for fat tissue, 0.957 for mucosa and 0.945 for muscle. The authors conclude that results are promising and future studies should consider in-vivo validation.

\citet{saito_nogueira_diffuse_2023} focuses on using diffuse reflectance spectroscopy (DRS) to guide colorectal cancer (CRC) in real-time through tissue characterization and identifying biomarkers. The goal is to improve surgical precision by detecting cancer margins and enhancing circumferential resection margin (CRM) determination, thereby reducing cancer recurrence and improving patient outcomes. A total of 2949 spectra were collected from 47 patients and a Classification and Regression Tree (CART) algorithm was used to classify normal, fat, and tumour tissues. Chromophores were extracted from the raw spectra and used as input for the classification. Measurements were taken at two different depths; 630 µm and 2500 µm to assess the extent to which probing depth would affect classification accuracy. The 630 µm probe achieved accuracies of 90.2\% (0.959 sensitivity, 0.989 specificity and 0.955 AUC). The 2500 µm probe reached an accuracy of 94\% (0.969 sensitivity, 0.989 specificity and 0.967 AUC). The authors conclude that future in-vivo testing is necessary but results are encouraging. The potential benefits of this system include real-time and accurate tissue identification when tactile feedback is not available to surgeons.

\citet{saito_nogueira_improving_2022} aimed to enhance colorectal cancer detection by extending the wavelength range and tissue depth probed by DRS. The study used SVM to classify normal and cancerous colorectal tissues using 2889 DRS spectra from 47 patients. The probes tested different depths, with source-detector distances of 630 µm (probe 1) and 2500 µm (probe 2). Key outcomes showed that deeper tissue probing (probe 2) resulted in higher classification accuracy, with 96.1\% sensitivity and 95.7\% specificity. Polynomial SVM models outperformed Gaussian SVMs in most cases. The results indicate that deeper tissue layers yield more reliable colorectal cancer detection metrics. The authors conclude that extending the wavelength range and probing deeper tissue layers significantly improves colorectal cancer detection. These findings suggest the potential of integrating DRS into colonoscopy tools, which could reduce unnecessary biopsies, improve cancer margin delineation, and ultimately enhance patient survival.

\citet{geldof_diffuse_2023} developed and assessed the feasibility of a compact side-firing optical fibre probe for real-time tissue discrimination during colorectal cancer surgery using DRS. The goal was to enhance tumour detection and surgical precision in hard-to-reach areas like the pelvis, where conventional flat-tipped fibre probes struggle to operate. The system was validated in Monte Carlo simulations, phantom studies, and ex-vivo measurements from colorectal cancer specimens. The side-firing probe’s performance was compared with flat-tipped probes in terms of light behaviour, measurement depth, and tissue classification accuracy. An SVM was used to classify DRS spectra. The authors found that side-firing fibres had reduced signal strength and measurement depth compared to flat-tipped fibres, but still provided accurate tissue classification. The side-firing probe achieved 92\% accuracy, 92\% sensitivity, and 96\% specificity in distinguishing tumours from healthy tissues. The study concluded that the side-firing DRS probe is a feasible solution for intraoperative tissue sensing, particularly in narrow spaces, with the potential for future integration into colorectal and laparoscopic surgeries.

\citet{nogueira_tissue_2021} aimed to differentiate between mucosa and tumour tissues based on tissue parameters extracted from DRS spectra. Data was collected from 47 subjects over the range of 350-1900 nm. A CART algorithm was implemented and the most important parameters for colorectal cancer classification were found to be total lipid content, reduced scattering amplitude and Mie scattering power. Two probing depths were tested and both achieved AUC values above 0.9. Probe 1 achieved 87.1\% sensitivity, 89.7\% specificity, 88.3\% accuracy and 0.915 AUC, whereas probe 2 achieved 81.8\% sensitivity, 88.2\% specificity, 84.8\% accuracy, and 0.90 AUC. The authors conclude that the extracted parameters are relevant for cancer identification in the colorectal lumen. In addition, they argue that they solved the quantification of independent tissue biochemical and microstructural parameters on superficial and deeper tissue layers without restrictions of diffusion theory and at an extended DRS wavelength range.

\citet{baltussen_using_2020} tested whether DRS signals could differentiate tumour tissues from fibrosis in resection specimens of advanced rectal cancer patients. 117 spectra were collected from 38 patients in the wavelength range 400 - 1700 nm. An SVM was implemented for classification. When differentiation of pure tumours from pure fibrosis measurement, accuracies of 0.88 were achieved (Specificity = 0.86, Sensitivity = 0.91, MCC = 0.76). However, if classification is completed on a mixture of healthy tissue with tumours the mean classification accuracy drops to 0.61 (Specificity = 0.66, Sensitivity = 0.51, MCC = 0.17). As such, the authors conclude that the main challenge for DRS is to detect tumours in a mixture of tumour and fibrosis tissues.

\section{Breast Cancer}



\citet{majumder_comparison_2008} compare the efficacy of autofluorescence, diffuse reflectance, combined fluorescence and diffuse reflectance, and Raman spectroscopy in classifying breast tissues into histopathological categories: invasive ductal carcinoma (IDC), ductal carcinoma in situ (DCIS), fibroadenoma (FA), and normal tissues. The study used 74 breast tissue samples to evaluate and compare these optical techniques based on spectral data acquired from ex vivo tissue samples. A logistic regression algorithm was developed for multiclass classification using spectral features. DRS achieved a classification accuracy of 51\% for invasive carcinoma, 28\% for ductal carcinoma in situ, 85\% for fibroadenoma and 86\% for normal breast tissue. The authors found that Raman spectroscopy outperformed the other methodologies for the task and concluded that Raman spectroscopy is superior for precise breast tissue classification, but combined fluorescence and diffuse reflectance holds potential for real-time clinical applications, such as evaluating tumour margins during surgery.

\citet{nachabe_diagnosis_2011} evaluated diffuse optical spectroscopy for diagnosing breast cancer. The study examines breast tissue spectra in the wavelength range of 500 to 1600 nm to discriminate between five types of breast tissues: adipose, glandular, fibroadenoma, invasive carcinoma (IC), and ductal carcinoma in situ (DCIS). The method extracts important tissue properties like blood, water, lipid, collagen, and scattering parameters. Using a classification and regression tree (CART) algorithm, the study achieved high sensitivity-specificity for tissue discrimination: 98-99\% for adipose, 84-95\% for glandular, 81-98\% for fibroadenoma, 91-95\% for IC, and 83-99\% for DCIS. The overall diagnostic performance was 94\%. The conclusion highlights diffuse optical spectroscopy as a promising tool for breast cancer diagnosis, with lipid proving to be a better discriminator for adipose tissue than beta-carotene. It recommends further investigation of diffuse optical spectroscopy for in vivo applications and suggests that lipid content is the most reliable indicator for classifying adipose tissue.

\citet{soares_diagnostic_2013} investigates the use of DRS to detect breast lesions with microcalcifications, which are critical for breast cancer diagnosis. Current methods, such as stereotactic core needle biopsy, miss microcalcifications in 15\% of cases, leading to non-diagnostic results and repeat procedures. The methods involved acquiring diffuse reflectance spectra from 203 sites on breast biopsy tissues from 23 patients. Using an SVM, the spectra were analyzed to differentiate normal tissue, lesions with microcalcifications, and lesions without microcalcifications. The outcomes showed high diagnostic power, with a positive predictive value (PPV) of 97\% and a negative predictive value (NPV) of 88\%. The sensitivity was 67\%, and the specificity was 99\%. The paper concludes that DRS is an effective tool for real-time detection of microcalcifications during biopsy, offering significant advantages in improving biopsy accuracy and reducing repeat procedures.

\citet{veluponnar_margin_2024} aimed to assess the diagnostic accuracy of DRS for the binary discrimination of healthy and tumorous breast tissue in up to 2mm depth. Data was collected both ex- and in-vivo. Models were trained on both datatypes and performance was evaluated on the in-vivo data. The best type of training data (ex-vivo only, in-vivo only or mixed) was evaluated. The implemented models were linear and quadratic sull, a weighted KUN and a gradient boosting model. The best performance was achieved by the gradient boosting model (RUSboost) when trained on both in- and ex-vivo data as opposed to just one data type. The algorithm achieved a MCC value of 0. 76. The authors conclude that DRS allows real-time margin assessment with high sensitivity and specificity during breast-conserving surgeries.

\citet{de_boer_towards_2018} investigated the use of an optical biopsy needle with integrated DRS for the in-vivo discrimination of healthy and malignant breast tissue. Spectra were collected from 32 patients undergoing ultrasound-guided breast biopsy. A total of 1100 wavelengths were collected between 500-1600hm. Feature selection was implemented, reducing the number of wavelengths to 8 and an SVM was used for classification. An accuracy of 93\% was achieved (UCC = 0.87, specificity = 0.91, sensitivity = 0.95). The authors conclude that DRS is feasible for integration in a surgical tool that could assist in detecting positive resection margins during breast surgery.

\citet{veluponnar_diffuse_2023}

Investigate different numbers of fibres for fiber-optic DRS 
Binary classification 
1200 features 
1770 instances 
normalisation + Feature extraction 
Gradient boosting model CRUS Boost)
Best performance at least 3 emitting fibres 
Accuracy varied w. tumor percentage, tumor - margin distance + number of fibres 
↳ from 75-1001. accuracyVeloponnar 2023

\citet{zhu_use_2005}
Single fibre optic probe for breast cancer detection 
during core needle biopsy. 
2 classes 
SVM
Accuracy of 85. 111. using outer ring (100\% spec, 46.15 Sens)

\citet{chaudhry_breast_2023}
Use DRS for binary classification using an extended-wavelength range 
Test Ew advantage standard range
PCA 
1035 instances 
LDA + SVM 
Sens 0. 94 + Spec. 0.91 for EW
Sens 0.40 and spec 0. 71 for standard
Ew better than the standard

\citet{evers_diffuse_2013}
47 patients for patient-wise comparison of malignant + healthy breast tissue 
Collective analysis 90 sens, 88 spec, 89 accuracy 
Per patient almost 100 \% 
CART 
Binary analysis 
Feature extraction for constituents

\citet{zhu_diagnosis_2006}
DRS in ultraviolet - visual spectrum 
Two models for feature selection ↳ Monte Carlo + patial- least squares 
Binary classification 
SVM @diffenet feature numbers 
79 ACC, 76-78 Spec., 83 Sens

